Drift Chamber Track Reconstruction for the P349 Antiproton Experiment

The aim of this thesis was to perform the drift chamber calibration and charged particles 3d track reconstruction for the P349 antiproton polarization experiment. A dedicated procedures were designed, implemented and tested on the experimental data for the the D1 drift chamber. The calibration consisted of the drift time offsets determination, estimation of the initial drift time - space relations by means of the homogeneous irradiation method and the iterative procedure for the time - space relations optimization. Calibration curves for all wire planes of the detector were determined. The obtained uncertainties of the hit position reconstruction are in the range of 150 - 220 $\rm \mu m$. Furthermore, based on the prepared 3d track reconstruction angular distribution of tracks passing through the drift chamber were determined.

==> Introduction.tex <==
\chapter{Introduction} \label{chapt:introduction}
